Fast View Synthesis with Deep Stereo Vision

Novel view synthesis is an important problem in computer vision and graphics. Over the years a large number of solutions have been put forward to solve the problem. However, the large-baseline novel view synthesis problem is far from being "solved". Recent works have attempted to use Convolutional Neural Networks (CNNs) to solve view synthesis tasks. Due to the difficulty of learning scene geometry and interpreting camera motion, CNNs are often unable to generate realistic novel views. In this paper, we present a novel view synthesis approach based on stereo-vision and CNNs that decomposes the problem into two sub-tasks: view dependent geometry estimation and texture inpainting. Both tasks are structured prediction problems that could be effectively learned with CNNs. Experiments on the KITTI Odometry dataset show that our approach is more accurate and significantly faster than the current state-of-the-art. The code and supplementary material will be publicly available. Results could be found here https://youtu.be/5pzS9jc-5t0

==> tables.tex <==
%\begin{table}[h!]
%\centering
%\caption{SSIM versus L1 distance}
%\label{table:l1versusssim}
%\begin{tabular}{|l|l|l|l|l|}
%\hline
%\multicolumn{2}{|l|}{}                                                         & Test 80       & Test 160      & Test 240       \\ \hline
%\multirow{2}{*}{Train 80}  & L1                                                & \textbf{6.66} & \textbf{8.90} & \textbf{12.14} \\ \cline{2-5} 
%                           & \begin{tabular}[c]{@{}l@{}}SSIM\\ L1\end{tabular} & 6.68          & 9.18          & 12.67          \\ \hline
%\multirow{2}{*}{Train 160} & L1                                                & \textbf{6.92} & \textbf{8.47} & \textbf{10.38} \\ \cline{2-5} 
%                           & \begin{tabular}[c]{@{}l@{}}SSIM\\ L1\end{tabular} & 7.22          & 8.66          & 10.63          \\ \hline
%\multirow{2}{*}{Train 240} & L1                                                & \textbf{7.47} & \textbf{8.73} & \textbf{10.28} \\ \cline{2-5} 
%                           & \begin{tabular}[c]{@{}l@{}}SSIM\\ L1\end{tabular} & 7.73          & 9.01          & 10.63          \\ \hline
%\end{tabular}
%\end{table}
%
%\begin{table}[h!]
%\centering
%\caption{Unet Architecture}
%\begin{tabular}{|l|l|l|l|}
%\hline
%\multicolumn{1}{|c|}{\textbf{}}                             & Test 80 cm & Test 160 cm & Test 240 cm \\ \hline
%\begin{tabular}[c]{@{}l@{}}Trained on\\  80 cm\end{tabular} & 7.12       & 9.34        & 11.99       \\ \hline
%\begin{tabular}[c]{@{}l@{}}Trained on\\ 160 cm\end{tabular} & 7.37       & 9.038       & 11.02       \\ \hline
%\begin{tabular}[c]{@{}l@{}}Trained on\\ 240 cm\end{tabular} & 7.75       & 9.16        & 10.85       \\ \hline
%\end{tabular}
%\end{table}
